Policy Mirror Descent Inherently Explores Action Space

Explicit exploration in the action space was assumed to be indispensable for online policy gradient methods to avoid a drastic degradation in sample complexity, for solving general reinforcement learning problems over finite state and action spaces. In this paper, we establish for the first time an $\tilde{\mathcal{O}}(1/\epsilon^2)$ sample complexity for online policy gradient methods without incorporating any exploration strategies. The essential development consists of two new on-policy evaluation operators and a novel analysis of the stochastic policy mirror descent method (SPMD). SPMD with the first evaluation operator, called value-based estimation, tailors to the Kullback-Leibler divergence. Provided the Markov chains on the state space of generated policies are uniformly mixing with non-diminishing minimal visitation measure, an $\tilde{\mathcal{O}}(1/\epsilon^2)$ sample complexity is obtained with a linear dependence on the size of the action space. SPMD with the second evaluation operator, namely truncated on-policy Monte Carlo (TOMC), attains an $\tilde{\mathcal{O}}(\mathcal{H}_{\mathcal{D}}/\epsilon^2)$ sample complexity, where $\mathcal{H}_{\mathcal{D}}$ mildly depends on the effective horizon and the size of the action space with properly chosen Bregman divergence (e.g., Tsallis divergence). SPMD with TOMC also exhibits stronger convergence properties in that it controls the optimality gap with high probability rather than in expectation. In contrast to explicit exploration, these new policy gradient methods can prevent repeatedly committing to potentially high-risk actions when searching for optimal policies.

==> application.tex <==
%!TEX root = ./exploration_free_pmd.tex

%%\subsection{TOMC with Multiple Trajectories -- Applications}\label{subsec_application_multi_traj}
%\yan{Feb 17, applications, also illustrating the importance of divergence}
%%We now specialize the generic convergence results of SPMD, developed in Section \ref{subsec_exp_multiple_traj_analysis}, to concrete Bregman divergences.
%In view of Theorem \ref{global_convergence_generic}, it suffices to determine $(\mu, \cD, \tau(\cD))$ for the divergence of~interest.
%%En route, we verify that Condition \ref{divergence_condition_fixed_optimal} indeed holds for the  Bregman divergences of interest.
%
%\begin{proposition}[Kullback–Leibler Divergence]\label{prop_kl}
%%Let $w(\pi(\cdot|s)) \coloneqq \tsum_{a \in \cA} \pi(a|s) \log \pi(a|s)$ for $\pi(\cdot|s) \in \mathrm{ReInt}(\Delta_{\cA})$,
%%and we extend its domain to $\Delta_{\cA}$ by defining $0 = 0 \log 0$.
%%Then $D^{\pi}_{\pi'}(s) = \tsum_{a \in \cA} \pi(a|s) \log (\tfrac{\pi(a|s)}{\pi'(a|s)})$ corresponds the Kullback–Leibler (KL) divergence between  $\pi(\cdot|s)$ and $\pi'(\cdot|s)$.
%For SPMD with KL divergence, one can take
%\begin{align*}
%\mu = 1, ~ \cD = 2 \log \abs{\cA}, ~ \tau(\cD) = \abs{\cA}^{-2/(1-\gamma)}.
%\end{align*} 
%%Consequently, 
%%suppose Assumption \ref{assump_unif_mixing} holds,
%%let $Q^{\pi_t, \xi_t}$ be constructed as in \eqref{eq_truncate_q}, with $(m,n)$ specified as \eqref{choice_m_n_general} and $\tau = \tau(\cD)$,
%
%Suppose 
%Assumption \ref{assump_unif_mixing} holds,
%the total number of iterations $k$ is given a priori, and 
% we construct $Q^{\pi_t, \xi_t}$  as in \eqref{eq_truncate_q}, with 
%$\tau =  \abs{\cA}^{-2/(1-\gamma)}$, and 
%\begin{align*}
%m = \Theta \rbr{\tfrac{\abs{\cA}^2}{(1-\gamma)^2 \varepsilon^2} \log (\tfrac{2 \abs{\cZ} k }{\delta}) },
%n = \tilde{\Theta} \rbr{
%\rbr{
%\tfrac{1}{1-\gamma} + \tfrac{ t_{\mathrm{mix}}}{\underline{\nu}} \abs{\cA}^{2/(1-\gamma)}} \log (\tfrac{\abs{\cA} }{\varepsilon})
%}, ~\text{with} ~ \varepsilon = \tfrac{M}{2} \sqrt{\tfrac{\cD}{\mu k }} ,
%\end{align*}
%where $ t_{\mathrm{mix}} =  \ceil{\log_\rho(\underline{\nu}/(2C)) - 2 \log_\rho (\abs{\cA} ) / (1-\gamma) }$,  $M = \tfrac{1}{1-\gamma}$,
%and $\delta \in (0,1)$.
%
%Setting $\eta  =  \sqrt{\tfrac{ \log \abs{\cA} }{2 k M^2} }$ in SPMD,  
%then with probability $1-\delta$, SPMD satisfies  
%\begin{align}\label{spmd_optimality_gap_kl}
%f(\hat{\pi}_k) - f(\pi^*)
%\leq 
%\tfrac{3 M }{1-\gamma} \sqrt{ \tfrac{2 \log \abs{\cA}}{ k}},
%\end{align}
%where $f(\hat{\pi}_k) = \min_{0 \leq t \leq k-1} f(\pi_t)$.
%In addition, for $\hat{\pi}_k$ to be an $\epsilon$-optimal policy, the total number of samples  is bounded by 
%\begin{align}\label{spmd_total_samples_kl}
%\tilde{\cO} \rbr{
%\tfrac{ \abs{\cA}^2 \log \abs{\cA}}{(1-\gamma)^6  \epsilon^4}
%\rbr{
%\tfrac{1}{1-\gamma} + \tfrac{ t_{\mathrm{mix}}}{\underline{\nu}} \abs{\cA}^{2/(1-\gamma)}}
%\log (\tfrac{36 \abs{\cZ}  \log \abs{\cA}}{\delta (1-\gamma)^4})
%\log (\tfrac{\abs{\cA}}{\epsilon})
%}.
%\end{align}
%\end{proposition}
%
%\begin{proof}
% $\mu = 1$ directly comes from the strong convexity of $w(\cdot)$ w.r.t $\norm{\cdot}_1$ norm, and $\cD = 2 \log \abs{\cA}$ follows from  $D^{\pi}_{\pi_0}(s) \leq \log \abs{\cA}$ when $\pi_0$ is the uniform policy.
%It remains to characterize $\tau(\cD)$.
%
%%Note that $\pi_t(a|s) \in \mathrm{ReInt}(\Delta_{\cA})$.
%%For any $s \in \cS$, 
%%and any $a^* \in \cA^*_s$, 
%%let $\pi^*$ be an optimal policy with $\pi^*(a^*|s) = 1$. 
%For any $\pi^* \in \overline{\Pi}^*$ and any $\pi \in \mathrm{ReInt}(\Pi)$,   $(1-\gamma) D^{\pi^*}_{\pi} (s)  \leq   \cD$ is equivalent to 
%\begin{align*}
%D^{\pi^*}_{\pi}(s) = \tsum_{a \in \cA} \pi^*(a|s) \log (\tfrac{\pi^*(a|s)}{\pi(a|s)}) 
%= - \log \pi(a^{\pi^*}_s |s) \leq \tfrac{2 \log \abs{\cA}}{1-\gamma},
%\end{align*}
%which implies $\pi(a^{\pi^*}_s|s) \geq \abs{\cA}^{-2/(1-\gamma)}$.
%Hence one can take $\tau(\cD) = \abs{\cA}^{-2/(1-\gamma)}$.
%%Now since $a^* \in \cA^*_s$ is arbitrary, this immediately implies $\tau(\cD) \geq \abs{\cA}^{-2/(1-\gamma)}$ and hence Condition \ref{divergence_condition_fixed_optimal} holds.
%Finally, plugging the choice of $(\mu, \cD, \tau(\cD))$ into Theorem \ref{global_convergence_generic} completes the proof.
%\end{proof}
%
%
%%Note that the update \eqref{spmd_update} of SPMD with $D^{\pi}_{\pi'}$ being the KL divergence admits a closed-form expression:
%%\begin{align*}
%%\pi_{k+1}(a|s) \propto \pi_k(a|s) \exp \rbr{ - \eta_k Q^{\pi_k, \xi_k}(s, a)}, ~\forall (s,a) \in \cS \times \cA.
%%\end{align*}
%%This also coincides with that of the stochastic variant of natural policy gradient method (SNPG) \cite{kakade2001natural}.
%It might be worth stressing that even though SPMD with KL divergence  yields an $\cO(\cH_{\cD} /\epsilon^4)$ sample complexity. 
%We have the constant $\cH_{\cD} = \Omega(\abs{\cA}^{-2/(1-\gamma)}$, which implies a sample complexity bound that can 
%have a very pessimistic polynomial dependence on the size of the action space, with the order being as large as the effective horizon $1/(1-\gamma)$.
%
%We next show that using the negative Tsallis entropy as the distance-generating function leads to a much improved dependence, on the  size of the action space and the effective horizon. 
%
%\begin{proposition}[Divergence induced by Negative Tsallis Entropy]\label{prop_tsallis}
%Let the distance-generating function 
%\begin{align}\label{dgf_tsallis}
%w(\pi(\cdot|s)) \coloneqq \tsum_{a \in \cA} - \pi(a|s)^p
%\end{align}
% in \eqref{def:kl_bregman}, for some $p \in (0,1)$.
%That is, $w$ corresponds to the negative Tsalli entropy with an entropy index $p$, up to a constant factor.
%In this case, we can take, with an additional subscript indicating the dependence on $p$, that
%\begin{align*}
%\mu_p = \tfrac{p (1-p)}{\abs{\cA}}, ~
%\cD_p = 2 ( \abs{\cA}^{1-p} - 1), ~
%\tau(\cD_p) = (\tfrac{2}{(1-\gamma) p})^{{1}/\rbr{p-1}} \abs{\cA}^{-1}.
%\end{align*}
%
%In particular,   suppose
%Assumption \ref{assump_unif_mixing} holds,
%and we choose $p = 1/2$ in \eqref{dgf_tsallis}.
%Let the total number of iterations $k$ be given a priori, and 
% let  $Q^{\pi_t, \xi_t}$ be constructed  as in \eqref{eq_truncate_q}, with 
%$\tau =  \rbr{{4}/\rbr{1-\gamma}}^{-2} \abs{\cA}^{-1}$, and 
%\begin{align*}
%m = \Theta \rbr{\tfrac{\abs{\cA}^2}{(1-\gamma)^2 \varepsilon^2} \log (\tfrac{2 \abs{\cZ} k }{\delta}) },
%n = \tilde{\Theta} \rbr{
%\rbr{
%\tfrac{1}{1-\gamma} + \tfrac{ t_{\mathrm{mix}}}{\underline{\nu} (1-\gamma)^2} \abs{\cA}} \log (\tfrac{\abs{\cA} }{\varepsilon})
%}, ~\text{with} ~ \varepsilon = \tfrac{M}{2} \sqrt{\tfrac{\cD}{\mu k }} ,
%\end{align*}
%where $ t_{\mathrm{mix}} = \ceil{\log_\rho (\underline{\nu}  (1-\gamma)^2 / (32C \abs{\cA}))}$,
%and 
%\begin{align*}
%\mu = \tfrac{1}{4\abs{\cA}}, ~
%\cD = 2 ( \abs{\cA}^{1/2} - 1), ~
%M = \tfrac{1}{1-\gamma},~
%\delta \in (0,1).
%\end{align*}
%Setting $\eta  =  \sqrt{\tfrac{ \abs{\cA}^{1/2} - 1 }{8 \abs{\cA}  k M^2} }$ in SPMD,  
%then with probability $1-\delta$, SPMD satisfies  
%\begin{align}\label{spmd_optimality_gap_tsallis}
%f(\hat{\pi}_k) - f(\pi^*)
%\leq 
%\tfrac{12 M }{1-\gamma} \sqrt{ \tfrac{\abs{\cA}^{3/2}}{ k}},
%\end{align}
%where $f(\hat{\pi}_k) = \min_{0 \leq t \leq k-1} f(\pi_t)$. 
%In addition, to find an $\epsilon$-optimal policy, the total number of samples required by SPMD is bounded by 
%\begin{align}\label{spmd_total_samples_tsallis}
%\tilde{\cO} \rbr{
%\tfrac{ \abs{\cA}^{7/2}}{(1-\gamma)^8  \epsilon^4}
%\rbr{
%\tfrac{1}{1-\gamma} + \tfrac{  t_{\mathrm{mix}} \cdot \abs{\cA}  }{\underline{\nu} (1-\gamma)^2}}
%\log (\tfrac{288 \abs{\cZ}  \abs{\cA}^{3/2}}{\delta (1-\gamma)^4  \epsilon^2})
%\log (\tfrac{\abs{\cA}}{\epsilon})
%}.
%\end{align}
%\end{proposition}
%
%\begin{proof}
%By definition, when the distance-generating function $w$ is specified as in \eqref{dgf_tsallis}, 
%\begin{align}\label{eq_divergence_tsallis}
%D^{\pi}_{\pi'}(s) =
%\tsum_{a \in \cA} - (\pi(a|s))^p + (1-p) \tsum_{a \in \cA} (\pi'(a|s))^p
%+ p \tsum_{a \in \cA} \pi(a|s) (\pi'(a|s))^{p-1}.
%\end{align}
%%Now take $\pi' = \pi_0$ as the uniform policy.
%%In addition, for any $s \in \cS$, 
%%and any $a^* \in \cA^*_s$, 
%%let $\pi^*$ be an optimal policy with $\pi^*(a^*|s) = 1$ for some $a^* \in \cA^*_s$, then
%For any $\pi^* \in \overline{\Pi}^*$, from \eqref{eq_divergence_tsallis} we obtain
%\begin{align*}
%D^{\pi^*}_{\pi_0} (s) =
% -1 + (1-p) \tsum_{a \in \cA} \abs{\cA}^{-p} + p \abs{\cA}^{-(p-1)} 
%= -1 + \abs{\cA}^{1-p},
%\end{align*}
%and hence one can take $\cD_p = 2 ( \abs{\cA}^{1-p} - 1)$.
%Meanwhile, $(1-\gamma) D^{\pi^*}_{\pi} \leq \cD_p$ implies 
%\begin{align*}
%(1-\gamma) ( p  \pi^{p-1}(a^{\pi^*}_s|s) -1) 
%\leq 2 ( \abs{\cA}^{1-p} -1 ),
%\end{align*}
%which in turn implies $\pi(a^{\pi^*}_s |s) \geq (\tfrac{2}{(1-\gamma) p})^{1/(p-1)} \abs{\cA}^{-1}$.
%Hence one can take $\tau(\cD_p) = (\tfrac{2}{(1-\gamma) p})^{1/(p-1)} \abs{\cA}^{-1}$,  and  Condition \ref{divergence_condition_fixed_optimal} holds.
%In addition, noting that $ - \tfrac{\partial^2}{\partial x^2} x^p  = p(1-p) x^{p-2} \geq p(1-p)$ for $x \in (0,1)$, we can take $\mu_p = \tfrac{p (1-p)}{\abs{\cA}}$.
%
%Finally, plugging the choice of $(\mu_p, \cD_p, \tau(\cD_p))$ with $p = {1}/{2}$ into Theorem \ref{global_convergence_generic} completes the proof.
%\end{proof}
%
%Comparing Proposition \ref{prop_kl} and \ref{prop_tsallis}, it is clear that the choice of divergence used in SPMD plays an important role in affecting the sample complexities. 
%In particular, using divergence induced by the negative Tsallis entropy yields a significantly better sample complexity than that of KL divergence, in terms of its dependence on the size of action space and the effective horizon.
%To the best of our knowledge, this seems to the first quantitative observation on the role of Bregman divergences for policy optimization methods in the stochastic RL setting.
%
%
%
%Note that update \eqref{spmd_update} of SPMD with $D^{\pi}_{\pi'}$ induced by the negative Tsallis entropy \eqref{dgf_tsallis} does not have a closed-form solution. 
%In this case, we show that  the subproblem \eqref{spmd_update} can be  solved to any accuracy in logarithmic number of steps,  via a simple bisection search subroutine.
%
%
%\begin{proposition}[Efficient Policy Update with Negative Tsallis Entropy]
%Consider SPMD update \eqref{spmd_update} with $D^{\pi}_{\pi'}$ induced by the negative Tsallis entropy \eqref{dgf_tsallis} with entropy index $p \in (0,1)$,  that is,
%\begin{align*}
%\textstyle
%%\label{spmd_update_tsalli}
%\pi_{k+1}(\cdot | s) = \argmin_{p(\cdot |s) \in \Delta_{\cA}} \eta_k \inner{Q^{\pi_k, \xi_k}(s, \cdot)}{p(\cdot|s)}   -
%\tsum_{a \in \cA}  (\pi(a|s))^p
%+ p \tsum_{a \in \cA} \pi(a|s) (\pi_k(a|s))^{p-1}.
%\end{align*}
% Define 
%$\psi_a(\mu) \coloneqq (\tfrac{p}{q_a - \mu})^{1/(1-p)}$, and 
%$\phi(\mu) \coloneqq \tsum_{a \in \cA}  \psi_a(\mu) - 1$, with $q_a \coloneqq \eta_k Q^{\pi_k, \xi_k}(s, a) + p \cdot (\pi_k(a|s))^{p-1}$ for every $a \in \cA$.
%In addition, let $l = \min_{a \in \cA} q_a - p \abs{\cA}^{1-p}$ and $h = \min_{a \in \cA} q_a - p$.
%Then
%\begin{align}\label{property_root_function}
%\phi ~\text{is strictly increasing on}~ [l, h], ~\text{and has a unique root}~ \mu^* \in [l, h].
%\end{align}
%
%Denote $\hat{\mu}^*$ the solution yielded by the standard root-finding bisection method \cite{ben2012optimization} applied to $\phi$ on $[l,h]$ for $B$ steps,
%and consequently define $\overline{x} \in \RR^{\abs{\cA}}$ as
%$
%\overline{x}_a =  \psi_a(\hat{\mu}^*)  / \tsum_{a'}  \psi_{a'}(\hat{\mu}^*)
%$
%for every $a \in \cA$.
%Then for any $\epsilon \in (0,1)$, we have 
%\begin{align}\label{tsallis_subproblem_num_steps}
%\overline{x} \in \mathrm{ReInt}(\Delta_{\cA}), ~ \text{and}~ \norm{\overline{x} - \pi_{k+1}(\cdot|s)}_\infty \leq \epsilon,
%\end{align}
%provided $B \geq \ceil{\log_2 (\tfrac{2 \abs{\cA}^2}{(1-p) \epsilon})}$.
%%In addition, the method requires only 
%%$ (B+3) \cdot \abs{\cA} $ number of scalar addition/multiplications.
%\end{proposition}
%
%
%\begin{proof}
%For Bregman divergence induced by the negative Tsallis entropy \eqref{dgf_tsallis}, given \eqref{eq_divergence_tsallis}, it is clear that update \eqref{spmd_update} for each state $s \in \cS$ is equivalent to the following optimization problem 
%\begin{align}\label{tsallis_update_problem}
%\textstyle
% \min_{x \in \RR^{\abs{\cA}}, x \geq \mathbf{0}}
%\inner{q}{x} - \tsum_{a \in \cA} x_a^p, ~ \text{s.t.} ~ \tsum_{a \in \cA} x_a = 1,
%\end{align}
%where $q_a = \eta_k Q^{\pi_k, \xi_k}(s, a) + p \cdot (\pi_k(a|s))^{p-1}$ for every $a \in \cA$.
%Noting that \eqref{tsallis_update_problem} satisfies the relaxed Slater condition, then we know that
%for an optimal solution $x^*$ to \eqref{tsallis_update_problem}, 
% there exists a  Lagrange multiplier $\mu^* \in \RR$, 
%\begin{align*}
%\textstyle
%x^* \in \Argmin_{x \in \RR^{\abs{\cA}}, x\geq \mathbf{0}}
%\inner{q}{x} - \tsum_{a \in \cA} x_a^p - \mu^*(\tsum_{a \in \cA} x_a - 1) .
%\end{align*} 
%The above problem is clearly separable, which implies 
%\begin{align*}
%\textstyle
%x^*_a \in \Argmin_{x_a \in \RR, x_a \geq {0}}
%q_a x_a -  x_a^p - \mu^* x_a  , ~ \forall a \in \cA.
%\end{align*}
%Since we know that $x_a^* \leq 1$, then one must have $\mu^* < \min_{a\in \cA} q_a$, since otherwise the above program as unbounded infimum with $x_a \to \infty$.
%In addition, since $p < 1$, we clearly have $x_a^* > 0$, and thus the first-order necessary optimality condition of the above program gives 
%\begin{align}\label{solution_primal_based_on_dual}
%q_a - p (x_a^*)^{p-1} - \mu^* = 0 ~\Rightarrow ~
%x_a^* = (\tfrac{q_a - \mu^*}{p})^{1/(p-1)}.
%\end{align}
%On the other hand, 
%from the Karush-Kuhn-Tucker condition, 
%we also know that any $x^*$ given by \eqref{solution_primal_based_on_dual} for some $\mu^* < \min_{a \in \cA} q_a$, while satisfying $\tsum_{a \in \cA} x_a^* = 1$ is an optimal solution to \eqref{tsallis_update_problem}.
%
%Now  plugging \eqref{solution_primal_based_on_dual} into constraint of \eqref{tsallis_update_problem} gives 
%$
%\tsum_{a \in \cA} (\tfrac{p}{q_a - \mu^*})^{1/(1-p)} = 1.
%$
%This implies that there must exists $a \in \cA$, such that $ (\tfrac{p}{q_a - \mu^*})^{1/(1-p)} \geq \tfrac{1}{\abs{\cA}}$, 
%and hence $\mu^* \geq q_a - p \abs{\cA}^{1-p} \geq \min_{a \in \cA} q_a - p \abs{\cA}^{1-p} $.
%In addition, for every $a \in \cA$, we have 
%$(\tfrac{p}{q_a - \mu^*})^{1/(1-p)} < 1$, and hence $\mu^* \leq \min_{a \in \cA} q_a - p$.
%Given our prior discussions, we see that 
%$\mu^* \in [l, h]$ with $l = \min_{a \in \cA} q_a - p \abs{\cA}^{1-p}$ and $h = \min_{a \in \cA} q_a - p$.
%
%In summary, we have identified that 
%\begin{align}\label{root_finding_formulation}
%\phi(\mu) \equiv \tsum_{a \in \cA}  (\tfrac{p}{q_a - \mu})^{1/(1-p)} - 1 ~ \text{has a solution $\phi(\mu^*) = 0$ with} ~ \mu^* \in [l,  h].
%\end{align}
%%Note that $\phi$ is strictly convex for $p \in (0,1)$. 
%%Given $[l, h]$, we then describe a bisection method that can find $\delta$-approximation of $\mu^*$ in $\cO(\log_2 (\tfrac{\abs{\cA}}{\delta}))$ number of iterations.
%
%Since $\phi'(\mu) = \sum_{a \in \cA} (q-1)  \tfrac{p^q}{(q_a - \mu)^{q+1}}  > 0$ for $\mu \in [l, h]$ and $q \coloneqq \tfrac{1}{1-p} > 1$.
%Hence $\phi$ is strictly increasing function on $[l, h]$,  with a unique root $\mu^* \in [l, h]$,
%and hence \eqref{property_root_function} is proved.
%Applying standard bisection method to $\phi$ on interval $[l, h]$ with $B$ iterations, we obtain $\hat{\mu}^* \in [l, h]$ with $\abs{\hat{\mu}^* - \mu^*} 
%\leq (h - l) 2^{-B} 
%\leq \abs{\cA} 2^{-B}$.
%
%Now define $\psi_a(\mu) = (\tfrac{q_a - \mu}{p})^{1/(p-1)}$, and let 
%$
%\hat{x}_a = \psi_a(\hat{\mu}^*)  , ~ x_a^* = \psi_a(\mu^*).
%$
%Note that both $\hat{x_a}, x_a^* > 0$ given that $\hat{\mu}^*, \mu^* \leq h \equiv \min_{a \in \cA} q_a - p$. 
%Define $\delta_a = \hat{x}_a - x_a^*$,  then from the mean value theorem 
%\begin{align*}
%\textstyle
%\abs{\delta_a} \leq \sup_{\mu \in [l, h]} \abs{\psi_a'(\mu)} \abs{\hat{\mu}^* - \mu^*}
%\leq \sup_{\mu \in [l, h]}  (q-1) \tfrac{p^q}{(q_a - \mu)^{q+1}}  \abs{\hat{\mu}^* - \mu^*}
%\leq \tfrac{1}{1-p}  \abs{\hat{\mu}^* - \mu^*},
%\end{align*}
%where in the last inequality we use again $ h \leq \min_{a \in \cA} q_a - p$.
%Given the above observation, let $\overline{x}_a = \hat{x}_a / \sum_{a' \in \cA} \hat{x}_a > 0$, 
%it is clear that $\overline{x} \in \mathrm{ReInt}(\Delta_{\cA})$.
%We then have 
%\begin{align*}
%\abs{ \overline{x}_a - x_a^*}  
%= \abs{
%\frac{x_a^* + \delta_a}{\tsum_{a'} (x_{a'}^* + \delta_a)} 
%-
%\frac{x_a^* }{\tsum_{a'} x_{a'}^* }  
%}
%=\abs{  \tfrac{\delta_a - x_a^* \sum_{a' \in \cA} \delta_{a'}}{1 + \sum_{a'} \delta_{a'}} }
%\leq \tfrac{\abs{\cA} \abs{\hat{\mu}^* - \mu^*} / (1-p)}{1 - \abs{\cA} \abs{\hat{\mu}^* - \mu^*} / (1-p)}
%\leq \tfrac{2 \abs{\cA}}{1-p} \abs{\hat{\mu}^* - \mu^*},
%\end{align*}
%provided $ \abs{\hat{\mu}^* - \mu^*} \leq (1-p) / (2 \abs{\cA})$.
%Now since $ \abs{\hat{\mu}^* - \mu^*} \leq \abs{\cA} 2^{-B}$, 
%we conclude that for any $\epsilon \in (0,1)$, to find $\abs{\overline{x}_a - x_a} \leq \epsilon$, it suffices let the number of iterations in the bisection procedure $B$ to satisfy
%$
%\tfrac{2 \abs{\cA}}{1-p} \cdot \abs{\cA} 2 ^{-B} \leq \epsilon.
%$
%Taking $B = \ceil{\log_2 (\tfrac{2 \abs{\cA}^2}{(1-p) \epsilon})}$  completes the proof for \eqref{tsallis_subproblem_num_steps}.
%%The total computation consists of: (1) forming $l$ and $h$; (2) evaluating $\phi(\cdot)$ at each Bisection step; (3) forming $\overline{x}$ in the end.
%%Each taking $\abs{\cA}$ unit computation. Hence the proof is completed.
%%The goal is to maintain a pair of iterates $l_t, h_t$ with $\phi(l_t) \leq 0 < \phi(h_t)$ for all $t \geq 0$.
%%Now suppose $(l_t, h_t)$ satisfies this condition for some iteration $t \geq 0$.
%%Then, if $\phi(l_t) = 0$, then we return $\mu^* = l_t$.
%%Otherwise $\phi(l_t) < 0$, and 
%%let us consider $m_t = \tfrac{l_t + h_t}{2}$. 
%%If $\phi(m_t) \leq 0$, then  we update $l_{t+1} = m_t$ and $h_{t+1} = h_t$.
%%If $\phi(m_t) > 0$, then we update $l_{t+1} = l_t$ and $h_{t+1} = m_t$.
%%It is clear that $\phi(l_{t+1}) \leq 0 < \phi(h_{t+1})$ by construction, and the interval length $\abs{h_t - l_t}$ decrease by a factor of $2$ at each iteration.
%%Hence in $\cO(\log_2 (\tfrac{\abs{\cA}}{\delta}))$ iterations one can find $\hat{\mu}^*$ with $\abs{\hat{\mu}^* - \mu^*} \leq \delta$.
%%
%%It remains to  find $l_0$ and $h_0$ such that 
%%$\phi(l_0) \leq 0 < \phi(h_0)$, or return a desired $\hat{\mu}^*$ with $\abs{\hat{\mu}^* - \mu^*} \leq \delta$.
%%Since $\phi$ is strictly convex, it is then impossible to have $\max \cbr{\phi(l), \phi(h)} < 0$,
%%since otherwise from convexity we have $\phi(u) < 0$ for any $u \in [l, h]$, contradicting with \eqref{root_finding_formulation}.
%%
%%If $\max \cbr{\phi(l), \phi(h)} = 0$, then we can safely return $\mu^* \in \cbr{l ,h}$ such that $\phi(\mu^*) = 0$.
%%On the other hand,
%%if $\max \cbr{\phi(l), \phi(h)} > 0$, then it suffices to choose $h_0$ with $\phi(h_0) = \max \cbr{\phi(l), \phi(h)}$, and 
%%$l_0$ with $\phi(l_0) = \min \cbr{\phi(l), \phi(h)}$ if $\min \cbr{\phi(l), \phi(h)} \leq 0$, otherwise let $l_0 = \argmin_{u \in [l,h]} \phi(u)$ which guarantees $\phi(l_0) \leq 0$ given \eqref{root_finding_formulation}.
%%On the other hand,
%%if $\max \cbr{\phi(l), \phi(h)} > 0$ and $\min \cbr{\phi(l), \phi(h)} \leq 0$,
%%then we can choose $l_0, h_0$ such that 
%%$\phi(l_0) = \min \cbr{\phi(l), \phi(h)}$ and  $\phi(h_0) = \max \cbr{\phi(l), \phi(h)}$.
%%
%%Finally, for the case when $\min \cbr{\phi(l), \phi(h)} > 0$.
%%For this case, it simply suffices to choose $l_0 = l$,
%\end{proof}
%

























